Developing Synthesis Flows Without Human Knowledge

Design flows are the explicit combinations of design transformations, primarily involved in synthesis, placement and routing processes, to accomplish the design of Integrated Circuits (ICs) and System-on-Chip (SoC). Mostly, the flows are developed based on the knowledge of the experts. However, due to the large search space of design flows and the increasing design complexity, developing Intellectual Property (IP)-specific synthesis flows providing high Quality of Result (QoR) is extremely challenging. This work presents a fully autonomous framework that artificially produces design-specific synthesis flows without human guidance and baseline flows, using Convolutional Neural Network (CNN). The demonstrations are made by successfully designing logic synthesis flows of three large scaled designs.

==> abstract.tex <==
\begin{abstract}

Design flows are the explicit combinations of design transformations, primarily involved in synthesis, placement and routing processes, to accomplish the design of Integrated Circuits (ICs) and System-on-Chip (SoC). Mostly, the flows are developed based on the knowledge of the experts. However, due to the large search space of design flows and the increasing design complexity, developing \textit{Intellectual Property (IP)-specific} synthesis flows providing high Quality of Result (QoR) is extremely challenging. This work presents a fully autonomous framework that artificially produces design-specific synthesis flows without human guidance and baseline flows, using Convolutional Neural Network (CNN). The demonstrations are made by successfully designing logic synthesis flows of three large scaled designs.

\end{abstract}

==> approach-old.tex <==
\section{Overview of Research Plan}

The overview of the proposed system is shown in Figure 3. It includes three major components: 

\subsection{Human-Inputs and Human-Operator}

Designers and EDA developers need to provide the required information and operations to initialize the system. For the designers, the design category (e.g., arithmetic datapath, ALU controller, etc.) and the design objectives (e.g., timing and area targets, power consumptions, etc.) are required. 


\begin{figure}[!htb]
\centering
\includegraphics[width=0.6\textwidth]{figs/overview.pdf}
\caption{Overview of the proposed autonomous system.}
\vspace{-4mm}
\label{fig:permutation}
\end{figure}

The baseline design flows are given by the EDA developers. The necessary constraints for ordering the EDA techniques are provided by them as well. For example, if an EDA function F1 has to be enabled by function F0, then F1 can only be placed after F0 in a design flow. The proposed system will try to discover better design flows, using the same set of functions used in the baseline flow. Alternatively, the EDA developers can let the system generate the top design flows with a given set of EDA techniques, without a baseline flow. The initial datasets should be given by the designers and the EDA developers. Informative datasets help the learning algorithms converge efficiently. The initial datasets will be generated by random flows (see Figures 2 and 3) if they are not available. In practice, the datasets and the EDA techniques could be updated anytime during the design process. Hence, the proposed system will accept the changes dynamically, as inputs of the online-learning modulo.

\subsection{Learning Components}

The learning components are the core of the proposed system. The IC design flow is an explicit combination of EDA techniques. These techniques are applied to the IC design iteratively. The design flows belong to winning flows class (or winning class), if they produce better design results than the baseline flow or the design objectives. For example, considering the timing constraint T, a design flow belongs to the winning class if it produces a design with delay less than T. The winning classes can be generalized with many design metrics such as delay, power, area, etc. The goal of these components is learning a classifier that forecast whether a design flow, i.e., a permutation of the EDA techniques, performs better another permutation. Finding the top design flows can be done by sorting a large number of permutations using the trained classifier. Specifically, there are three components implemented, i.e., offline learning, online learning and classifier finalization. 

Offline-learning techniques generate the best models by learning on the entire training data set at once. In the proposed system, offline learning component is used to learn the classifier with the static datasets. Offline learning techniques are usually not efficient if the datasets are too large. Fortunately, the size of the hardware design datasets is usually much smaller than other domains. However, this could affect the quality (accuracy of classification) of the trained model. Therefore, an online-learning modulo that updates the model with future dataset and changes of EDA tools is introduced in this system. Online-learning is a method of machine learning in which data becomes available in a sequential order and is used to update our best predictor for future data at each step, as opposed to offline-learning. The online-learning modulo will start when offline-learning finishes. If the static datasets are not provided, the offline-learning is initialized with random permutation testing (e.g., examples in Figure 2). The classifier is learned after a number of iterations of online-learning. 

\subsection{User Interface}

The user interface component aims to give the user-friendly solutions to the designers. It will first use the model learned by training, and find the solutions by doing classification permutation testing. This will allow us to test a larger number of permutations with affordable error rate. Finally, a small number of design flows will be delivered to the users. The accuracy of the trained classifier will be analyzed in this part. A mathematical model will be introduced for classification accuracy analysis with the user feedbacks.

